The Role of Linguistic Priors in Measuring Compositional Generalization of Vision-Language Models

Compositionality is a common property in many modalities including natural languages and images, but the compositional generalization of multi-modal models is not well-understood. In this paper, we identify two sources of visual-linguistic compositionality: linguistic priors and the interplay between images and texts. We show that current attempts to improve compositional generalization rely on linguistic priors rather than on information in the image. We also propose a new metric for compositionality without such linguistic priors.

==> ablation.tex <==
In this section, we will talk about the ablation studies about our proposed methods. The detailed results are shown in Table \ref{tab:hard-test-acc-full}.

\subsection{Number of Trials in Assist and Replace Methods}

In both our Assist and Replace methods, we randomly generate several candidates for the negative captions, and select the one with the lowest perplexity. The more candidates we generate for each true caption, the lower the perplexity will be. We choose to generate 10 or 30 random negative captions for Assist and 5 or 15 random negative captions for Replace, and the performance of the resulting models are not sensitive to the number of trials. This is because both Assist and Replace usually cannot decrease the perplexity of the original caption, and the perplexity difference between the generated negative caption and the original one will be stable as long as the number of trials is not too small. In the experiments, we choose 10 trials for Assist and 15 for Replacement, which yield slightly better results.

\subsection{Number of epochs in training}

We trained the model for 5 epochs, replicating the procedure of \citet{yuksekgonul2022and}. We also tested the performance of the other checkpoints, and found that the checkpoints from epoch 2 to epoch 4 always have performances between those of epoch 1 and 5. Comparing epoch 1 and 5, we notice that for most networks, epoch 1 has a better accuracy on the Ordering tasks and VG Attribution, which epoch 5 usually has better accuracies on VG Relation. This may reflect a change of focus and feature leaning/suppressing during the fine-tuning process. Since the ordering of the models usually don't change in terms of the number of epochs trained, we select to show the performance at epoch 5 for a fair comparison to \citet{yuksekgonul2022and}.

\subsection{Number of captions per image}

Each image in MSCOCO \cite{lin2014microsoft} usually has 5 captions, and we can choose to include all captions or only one of them during training. We tried both versions for CLIP variants, and found that the ranking of the models doesn't change for the two scales of training, although the models trained using 5 captions have clearly better accuracy. We choose to only keep the first caption for each image to speed up training, and we believe this doesn't influence the main results of our paper. The models trained with all captions are labeled ``large scale'' in the table.

\subsection{Number of words replaced}

In Replace methods, we can choose to replace more words, which could change the meaning of the caption by more and potentially further decrease the perplexity of the negative caption. We tried changing 2 words for each caption, and found that this can further increase the prediction accuracy for most tasks no matter whether we change 2 words of the same part of speech (POS) or not. The models with names containing ``2'' are these trained with 2 words replaced.

\subsection{Other ways of replacement: Language model assistance}

To improve the model's compositional generalization ability, we would like to select hard negative captions that are close to the original caption in words but different from the original caption in meaning. There are several ways of doing this. One could use a language model, e.g., BERT \cite{devlin2018bert}, to solve a cloze where the missing word is the word that we want to replace. One could also utilize the power of huge language models to generate the hard negatives by prompt engineering, and we use GPT-J-6B \cite{gpt-j} in the experiments. Both methods improve the performance of CLIP via fine-tuning, but the effect is worse than those of simple Assist and Replace methods.

==> improve.tex <==
To improve the comopositional generalization of CLIP, we propose several new methods to generate hard negatives during contrastive fine-tuning of CLIP.

\subsection{Experimental Settings}

Similar to \citet{yuksekgonul2022and}, we use the openCLIP \cite{ilharco_gabriel_2021_5143773} framework to fine-tune the CLIP \cite{radford2021learning} model. We use the ``ViT-B/32'' variant of CLIP with weights pre-trained by OpenAI. We use the training set of Karpathy split\footnote{https://github.com/karpathy/neuraltalk} for MSCOCO \cite{lin2014microsoft} dataset, and only keep the first caption for each image to speedup training. We use a batch size of 256, learning rate of 5e-6, and 50 steps of linear warmup with Cosine learning rate decay afterwards. We train 5 epochs in total.

\subsection{Reasons Why NegCLIP Overfits the Linguistic Prior}

We have shown in Section \ref{sec:NegCLIP} that the performance improvement of NegCLIP over CLIP and CLIP\_FT has a strong correlation with the linguistic prior. Note that the only difference between NegCLIP and CLIP\_FT is the existence of hard negative captions, the reason why NegCLIP overfits the linguistic prior must come from these negative captions. Since they are generated by swapping two random elements in the sentence, it is very likely that the negative caption has a much larger perplexity than the true caption.

After computing the perplexities of all captions in the training set of NegCLIP using AVG\_LM, we found that 98.93\% of the negative captions have higher average perplexity than the true caption, and in average the perplexities of negative captions is higher than that of the true caption by 1.72. Therefore, the model could easily distinguish the true caption from the negative captions by learning the linguistic prior. Since contrastive learning could lead the models to learn ``shortcut'' features \cite{robinson2021can} and the text encoders can learn word ordering information \cite{papadimitriou2022classifying}, models trained using NegCLIP would learn the linguistic prior purely from the text side. Besides, training for longer could even hurt the hard test accuracy of NegCLIP because it can overfit to the linguistic prior and hurt the other useful features.

To improve the compositional generalization ability of multi-modal networks, note that the compositional generalization performance consists of two parts, i.e., the uni-modal part and the multi-modal part. Thus, there are two ways for improvement: On the one hand, we could ``inject'' more linguistic priors into the network without hurting its hard negative accuracy. On the other hand, we could improve its interaction with the image side while preserving the linguistic prior. This simple idea leads to our two improvements to CLIP model, which we call CLIP\_Assist and CLIP\_Replace.

\begin{table}[t]
\caption{Example hard negative captions}
\label{tab:negative-example}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{ll}
\toprule
Method & Caption Example \\
\midrule
Original & a fire hydrant on a city street \\
\midrule
NegCLIP & a street hydrant on a city fire\\
CLIP\_Assist & a fire hydrant on a street city\\
CLIP\_Replace & a fire hydrant on a giraffe street\\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

\subsection{Assist: Improve Overall Accuracy}

To improve the accuracy of NegCLIP on ARO datasets, we could select negative samples with higher quality. Since the negative captions generated by randomly swapping two linguistic elements usually have high perplexities, we did multiple random trials and select the one with the lowest perplexity. This would make the negative captions harder to distinguish from the true caption. We name this method CLIP\_Assist because we utilize the assistance from language models to filter training data.

Since swapping two elements in a normal caption usually increases the perplexity, linguistic priors are still able to separate the negative captions from the true caption. An example of the caption generated using this method can be seen in Table \ref{tab:negative-example}. We could see that the negative sample for CLIP\_Assist makes more sense than that of NegCLIP, but is still less likely than the true caption.

The results of CLIP\_Assist is shown in Table \ref{tab:hard-test-acc-CLIP-variants}. Across all ARO datasets, most of its performances are better than NegCLIP, especially the overall accuracies. Therefore, by choosing negative captions that are harder for language models to classify, we could ``inject'' more linguistic priors into the CLIP model.

\begin{table*}[t]
\caption{Standard and Hard Test Accuracies for CLIP variants, shown in format ``overall accuracy / hard overall accuracy / hard test accuracy'' for VG Relation and ``overall acc/hard test acc'' for the other datasets. For each dataset, the highest accuracy is in bold, and the second highest is underlined.}
\label{tab:hard-test-acc-CLIP-variants}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccc}
\toprule
 & COCO\_Order & Flickr\_Order & VG Attribution & VG Relation \\
\midrule
CLIP & 47.73 / 43.56 & 59.12 / 48.70 & 61.35 / 57.92 & 59.79 / 53.52 / \textbf{55.90}\\
CLIP\_FT & 31.18 / 27.10 & 40.96 / 32.17 & 62.41 / 58.12 & 60.01 / 53.11 / \underline{50.48}\\
NegCLIP & \underline{91.74} / \underline{71.56} & 93.90 / 82.61 & 72.21 / 58.57 & \underline{80.50} / 60.94 / 48.62 \\
CLIP\_Assist & 91.46 / 71.41 & \underline{94.22} / \underline{83.48} & \underline{72.52} / 57.94 & \textbf{81.89} / \textbf{62.07} / 50.20 \\
CLIP\_Replace & 83.01 / 65.72 & 88.14 / 73.04 & 70.40 / \textbf{60.61} & 73.37 / 58.27 / 47.34 \\
\midrule
CLIP\_Double & \textbf{91.80} / \textbf{72.01} & \textbf{94.54} / \textbf{86.96} & \textbf{73.27} / \underline{59.38} & 80.33 / \underline{61.54} / 46.56\\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

\subsection{Replace: Improve Hard Test Accuracy}

The other way of improving the compositional generalization is to improve the interaction between the image and the captions. Besides, we want to prevent the model from taking the shortcut and only learning the linguistic prior from the hard negatives. Since swapping elements within true captions usually increases the perplexity, we replace a word in the true caption, which could potentially make the resulting caption become more probable but does not associate with the image. For instance, for the caption ``a man sitting at a table with a box of donuts.'' We could replace ``donuts'' with ``cookies'', and it will be hard to decide which one is the true caption without looking at the image. Therefore, replacing words in true captions can generate hard negatives that force the model to learn the alignment between the image and the captions.

In our experiments, we choose a random content word in the true caption, and replace it with another word with the same part of speech as the original word. We sample the new word from the distribution of words from the entire COCO caption dataset. We try multiple times and select the caption with the lowest perplexity among all random trials.

The experimental results can also be seen in Table \ref{tab:hard-test-acc-CLIP-variants}. CLIP\_Replace largely improves the hard test accuracy on VG Attribution dataset by choosing negatives that forces the model to look at the image. However, these negatives also hurt the linguistic priors in the resulting model, decreasing the accuracies of tasks that heavily requires linguistic priors, e.g., COCO Ordering and Flickr Ordering.

\subsection{Double: Combine Assist and Replace to Improve both accuracies}

Having improved the compositional generalization ability of CLIP in two different ways, one natural idea is to combine these two methods together. Therefore, we use negative captions from both CLIP\_Assist and CLIP\_Replace to fine-tune CLIP, and call the resulting model CLIP\_Double. As shown in Table \ref{tab:hard-test-acc-CLIP-variants}, CLIP\_Double improves both the overall accuracy and the hard negative accuracy over NegCLIP on most ARO datasets.
